Temporal Blind Spots in Large Language Models

Large language models (LLMs) have recently gained significant attention due to their unparalleled ability to perform various natural language processing tasks. These models, benefiting from their advanced natural language understanding capabilities, have demonstrated impressive zero-shot performance. However, the pre-training data utilized in LLMs is often confined to a specific corpus, resulting in inherent freshness and temporal scope limitations. Consequently, this raises concerns regarding the effectiveness of LLMs for tasks involving temporal intents. In this study, we aim to investigate the underlying limitations of general-purpose LLMs when deployed for tasks that require a temporal understanding. We pay particular attention to handling factual temporal knowledge through three popular temporal QA datasets. Specifically, we observe low performance on detailed questions about the past and, surprisingly, for rather new information. In manual and automatic testing, we find multiple temporal errors and characterize the conditions under which QA performance deteriorates. Our analysis contributes to understanding LLM limitations and offers valuable insights into developing future models that can better cater to the demands of temporally-oriented tasks. The code is available\footnote{https://github.com/jwallat/temporalblindspots}.

==> Figures/error_analysis/prompt_analysis_alpaca_archivalqa.tex <==
\begin{tikzpicture}
    \pie[text={pin}, radius=2, color={{rgb:red,69;green,125;blue,130}, {rgb:red,130;green,75;blue,108}, {rgb:red,62;green,130;blue,97}, {rgb:red,130;green,83;blue,49}, {rgb:red,60;green,130;blue,56}}]{51/Full sentence, 4/Answer artifact, 2/Repeated prompt, 11/No answer, 32/Good format}
\end{tikzpicture}


==> Tables/alpaca_prompt.tex <==
Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request.

### Instruction:
Answer the question.

### Input:
{davinci prompt}

### Response:

==> Tables/davinci_prompt.tex <==
\begin{lstlisting}[breaklines=true,tabsize=0]
I am a highly intelligent question answering bot. If you ask me a question that is rooted in truth, I will give you the answer. If you ask me a question that is nonsense, trickery, or has no clear answer, I will respond with 'Unknown'.

Q: What is human life expectancy in the United States?
A: 78 years

Q: Who was president of the United States in 1955?
A: Dwight D. Eisenhower

Q: Which party did he belong to?
A: Republican Party

Q: Where were the 1992 Olympics held?
A: Barcelona, Spain.

Q: {question}
A:
\end{lstlisting}

==> Tables/intro-example.tex <==
\begin{table}
    \center
    \small
    \makegapedcells
    \begin{tabular}{ll}
        \toprule
        
        & \makecell[l]{\texttt{Who loses WBA boxing title, refusing to fight} \\ \texttt{Tony Tucker in March 1995?}} \\
        
        \textsc{Alpaca} & \texttt{Mike Tyson}    \xmark{} Popularity error\\

        GT Ans. & \texttt{George Foreman} \\
        \midrule

        & \makecell[l]{\texttt{Which film won seven Oscars in 1994?}} \\
        
        \textsc{ChatGpt} & \texttt{Forrest Gump} \xmark{} Temporal hallucination: the movie won multiple Oscars in \textbf{1995}\\

        GT Ans. & \texttt{Schindler's List} \\
        
        \bottomrule
    \end{tabular}
    \caption{Examples of temporal blindspots (GT Ans indicates correct answer).}
    \label{tab:intro_example}
\end{table}


==> Tables/templama_overview.tex <==
\begin{table}[ht]
\scriptsize
\begin{tabular}{llcl}
\hline
\textbf{\textbf{ID}} & \textbf{\textbf{Relation}} & \textbf{\textbf{\#Qs}} & \textbf{\textbf{Template}}                                                                                    \\ \hline
P54                           & member of sports team      & 9033                         & \textless{}subject\textgreater~ played for which team in \textless{}year\textgreater{}?                 \\
P39                           & position held              & 7343                         & \textless{}subject\textgreater~ held which position in \textless{}year\textgreater{}?                         \\
P108                          & employer                   & 9049                         & \textless{}subject\textgreater~ worked for which company in \textless{}year\textgreater{}?                    \\
P102                          & political party            & 7324                         & \textless{}subject\textgreater~ was a member of which party in \textless{}year\textgreater{}?                 \\
P286                          & head coach                 & 4886                         & \textless{}object\textgreater~ was the head coach of which team in \textless{}year\textgreater{}?             \\
P69                           & educated at                & 1672                         & \textless{}subject\textgreater~ attended which university in \textless{}year\textgreater{}?                   \\
P488                          & chairperson                & 4190                         & \textless{}object\textgreater~ was the chair of which entity in \textless{}year\textgreater{}?                \\
P6                            & head of government         & 4125                         & \textless{}object\textgreater~ is the head of the government of which state in \textless{}year\textgreater{}? \\
P127                          & owned by                   & 2688                         & \textless{}subject\textgreater~ is owned by whom in \textless{}year\textgreater{}?                            \\ \hline
\end{tabular}
\caption{Overview of the TempLAMA relations and their reformulations to natural questions.}
\label{}
\end{table}
